Symmetry Breaking in the Congest Model: Time- and Message-Efficient Algorithms for Ruling Sets

We study local symmetry breaking problems in the CONGEST model, focusing on ruling set problems, which generalize the fundamental Maximal Independent Set (MIS) problem. A $\beta$-ruling set is an independent set such that every node in the graph is at most $\beta$ hops from a node in the independent set. Our work is motivated by the following central question: can we break the $\Theta(\log n)$ time complexity barrier and the $\Theta(m)$ message complexity barrier in the CONGEST model for MIS or closely-related symmetry breaking problems? We present the following results: - Time Complexity: We show that we can break the $O(\log n)$ "barrier" for 2- and 3-ruling sets. We compute 3-ruling sets in $O\left(\frac{\log n}{\log \log n}\right)$ rounds with high probability (whp). More generally we show that 2-ruling sets can be computed in $O\left(\log \Delta \cdot (\log n)^{1/2 + \varepsilon} + \frac{\log n}{\log\log n}\right)$ rounds for any $\varepsilon > 0$, which is $o(\log n)$ for a wide range of $\Delta$ values (e.g., $\Delta = 2^{(\log n)^{1/2-\varepsilon}}$). These are the first 2- and 3-ruling set algorithms to improve over the $O(\log n)$-round complexity of Luby's algorithm in the CONGEST model. - Message Complexity: We show an $\Omega(n^2)$ lower bound on the message complexity of computing an MIS (i.e., 1-ruling set) which holds also for randomized algorithms and present a contrast to this by showing a randomized algorithm for 2-ruling sets that, whp, uses only $O(n \log^2 n)$ messages and runs in $O(\Delta \log n)$ rounds. This is the first message-efficient algorithm known for ruling sets, which has message complexity nearly linear in $n$ (which is optimal up to a polylogarithmic factor).

==> prelim.tex <==

\paragraph{Computing Model} 
We consider a distributed network of $n$ nodes, modelled as an undirected graph $G$, where computation proceeds in synchronous rounds. 
In each round, every node can first perform some local computation including the access to a private source of randomness, and then nodes can exchange (possibly distinct) messages with each of their neighboring nodes according to the topology defined by $G$.
As we are interested in algorithms that are scalable to large networks, we assume that the size of a message is bounded by $O(\log n)$ bits, which corresponds to the standard CONGEST model~\cite{PelegBook}.
Each node is equipped with a unique ID chosen from a range polynomial in $n$, but nodes do not possess any other prior knowledge about the network topology at large.



